Multitask-based Evaluation of Open-Source LLM on Software Vulnerability

This paper proposes a pipeline for quantitatively evaluating interactive Large Language Models (LLMs) using publicly available datasets. We carry out an extensive technical evaluation of LLMs using Big-Vul covering four different common software vulnerability tasks. This evaluation assesses the multi-tasking capabilities of LLMs based on this dataset. We find that the existing state-of-the-art approaches and pre-trained Language Models (LMs) are generally superior to LLMs in software vulnerability detection. However, in software vulnerability assessment and location, certain LLMs (e.g., CodeLlama and WizardCoder) have demonstrated superior performance compared to pre-trained LMs, and providing more contextual information can enhance the vulnerability assessment capabilities of LLMs. Moreover, LLMs exhibit strong vulnerability description capabilities, but their tendency to produce excessive output significantly weakens their performance compared to pre-trained LMs. Overall, though LLMs perform well in some aspects, they still need improvement in understanding the subtle differences in code vulnerabilities and the ability to describe vulnerabilities to fully realize their potential. Our evaluation pipeline provides valuable insights into the capabilities of LLMs in handling software vulnerabilities.

==> sections/RQ4.tex <==

\subsection{\bf RQ-4: Evaluating Vulnerability Repair of ChatGPT}
 

% \xy{
% Addressing vulnerabilities in software systems is crucial for risk mitigation and software quality enhancement. Vulnerability Repair tasks require effective identification and remediation of these flaws within the codebase, which can help avert cyber-attacks and their potentially severe consequences, such as significant financial losses and endangering human lives. We want to examine ChatGPT's proficiency in efficiently repairing vulnerabilities in software systems.
% }


\noindent
\textbf{Setting.}
We instruct ChatGPT with the following prompts (i.e., Prompt 4.1 and Prompt 4.2) to tell it to repair vulnerable code: 1) providing ChatGPT with the vulnerable code to explore its performance (Prompt 4.1). 2) providing ChatGPT with vulnerable relevant lines when the vulnerable code exists to investigate the performance differences (Prompt 4.2). Table~\ref{tab:vr_example} show an example of how we investigate ChatGPT’s ability of vulnerability repair.



\noindent
\intuition{
\em{\textbf{Prompt 4.1}}: 
I will provide you with a vulnerable C code snippet and you must repair it. This C code snippet definitely has a vulnerability, so you don't need to determine whether there is a vulnerability, just output the repaired whole c code snippet without explanation.

\textbf{Prompt 4.2}: I will provide you with a vulnerable C code snippet and vulnerable lines, you must repair it. This C code snippet definitely has a vulnerability, so you don't need to determine whether there is a vulnerability. You need to use the index to label each line of code, and I will provide you with lines of code that are vulnerable such as Lines: [1, 4, 5], just output the repaired whole c code snippet without explanation.
}



\noindent
\textbf{Results.}
Due to the hidden naturalness of vulnerabilities and the lack of context, it is difficult to determine whether ChatGPT has successfully fixed a vulnerability through manual observation. 
Therefore, when evaluating, we choose the code with \textit{only one line} of vulnerability and determine whether ChatGPT has fixed the vulnerable line and its contextual statements. 
If so, the performance metric \textit{Hit} is calculated as 1, indicating that it has the ability to fix the vulnerability. 
Otherwise, the \textit{Hit} is assigned with 0.
Table~\ref{tab:chatgpt-vr-cwe} displays detailed results on how ChatGPT performs on Top-10 CWE types. 
The \textit{Hit} metric indicates whether ChatGPT successfully fixes the vulnerable line, while \textit{Hit$_{ctx}$} means the ChatGPT's performance provided with additional context information (i.e., the vulnerable relevant  lines).
Finally, the column ``\# Manual'' means the number of patches correctly generated by ChatGPT when we manually compare it with the ground truth.


Based on the table, we can make the following observations:
\begin{itemize}[leftmargin=*]
    \item Overall, ChatGPT shows limited success in repairing vulnerable code snippets, with an average Hit rate of 0.2 and Hit$_{ctx}$ of 0.24. This suggests that there is room for improvement in its ability to detect and fix vulnerabilities.
    \item The performance of ChatGPT varies across different CWE types. For some types, like CWE-264, it has a perfect score (1) in both Hit and Hit$_{ctx}$, while for others, like CWE-476 and CWE-119, it fails to fix the vulnerability altogether.
    \item Providing vulnerable lines (Prompt 4.2) does not consistently improve ChatGPT's performance. For some CWE types, the Hit$_{ctx}$ is higher than the Hit rate (e.g., CWE-189), while for others, it remains the same or decreases (e.g., CWE-20). This indicates that the extra information may not always be helpful for ChatGPT in repairing the vulnerability.
    \item ChatGPT has the trivial ability to repair a vulnerability.
\end{itemize}


% \chao{add analysis to the TWO instances which are correctly repaired}

% \find{
% \textbf{Finding-8}: ChatGPT's performance in vulnerability repair varies across different CWE types, with an average Hit score of 0.2 and Hit$_{idx}$ score of 0.24. The model demonstrates better performance in some categories, like CWE-264, while struggling in others, like CWE-476 and CWE-362. The providing of vulnerable lines (Prompt 4.2) does not always lead to improved performance, indicating that there is still room for improvement in ChatGPT's ability to repair vulnerabilities.
% }

\find{
\textbf{Finding-8}: ChatGPT has limited ability in repairing vulnerability no matter when provided with context information or not.
}

% \xy{
We also delve into the specific information of CWE types to analyze ChatGPT's performance:
\begin{itemize}[leftmargin=*]
    \item \textbf{CWE-264 (Privilege Escalation).} ChatGPT performs well in fixing vulnerabilities related to privilege escalation, with a perfect score of 1 in both hit and hit$_{ctx}$. This could be because privilege escalation vulnerabilities often involve specific patterns, such as incorrect permission checks or improper use of privileges, which the ChatGPT might have learned effectively during training.
    
    \item \textbf{CWE-476 (NULL Pointer Dereference) and CWE-119 (Improper Restriction of Operations within the Bounds of a Memory Buffer).} 
    ChatGPT struggles to fix these vulnerabilities even find no vulnerable position, resulting in a hit and hit$_{ctx}$ score of 0. 
    These types of vulnerabilities might be more challenging for the ChatGPT due to their complex naturalness and dependence on the specific context of the code. For instance, detecting and fixing a NULL pointer dereference often requires understanding the control flow and data flow of the code, while buffer-related vulnerabilities require a deep understanding of memory management.
    
    \item \textbf{CWE-189 (Numeric Errors) and CWE-125 (Out-of-bounds Read).} 
    ChatGPT's performance varies for these types, with hit scores of 0.17 and 0.2, and hit$_{ctx}$ scores of 0.5 and 0.2, respectively. This suggests that the ChatGPT might have some understanding of the patterns involved in these vulnerabilities, but its success in fixing them is inconsistent. Numeric errors often involve incorrect calculations or data conversions, while out-of-bounds read issues typically stem from improper boundary checks. Improving ChatGPT's understanding of these patterns and their underlying causes could potentially enhance its performance in repairing these vulnerabilities.
\end{itemize}


\find{
\textbf{Finding-9.}
ChatGPT's performance in repairing different CWE types can be attributed to its ability to recognize and understand specific vulnerability patterns. 
For certain types with well-defined patterns, it performs well, while for others with more complex or context-dependent patterns, it struggles to identify and fix the vulnerabilities. 
% Enhancing the ChatGPT's understanding of these complex patterns, control flows, and data flows could potentially improve its overall performance in repairing code vulnerabilities.
}





% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Examples of Vulnerability Repair}
 % \resizebox{1\linewidth}{!}
 {
    \begin{tabular}{|l|p{36.085em}|}
    \hline
    \textbf{Setting} & \cellcolor[rgb]{ .957,  .847,.855}\textbf{Vulnerable Code} \\
    \hline \hline

    \textbf{Prompt} & {\cellcolor[rgb]{ .851,  .882,  .949}\textit{I will provide you with a vulnerable C code snippet and you must repair it. This C code snippet definitely has a vulnerability, so you don't need to determine whether there is a vulnerability, just output the repaired whole c code snippet without explanation.}}
    \\ \hline
    
    \textbf{Input} & \multicolumn{1}{p{29.75em}|}{
    An example of a C code snippet with vulnerabilities (CVE-2019-17773).} 
    \\ \hline \hline
    
    \textbf{Setting} & \cellcolor[rgb]{.902,1,.925} \multicolumn{1}{l}{\textbf{Vulnerable Code} \& \textbf{Vulnerable relevant lines}} \\
    \hline \hline

   \textbf{Prompt} &  {\cellcolor[rgb]{ .851,  .882,  .949}\textit{I will provide you with a vulnerable C code snippet and vulnerable lines, you must repair it. This C code snippet definitely has a vulnerability, so you don't need to determine whether there is a vulnerability. You need to use the index to label each line of code, and I will provide you with lines of code that are vulnerable such as Lines: [1, 4, 5], just output the repaired whole c code snippet without explanation.}} 
    \\ \hline
    
    \textbf{Input} & An example of a C code snippet with vulnerabilities (CVE-2019-17773). \newline{}Vulnerable relevant lines: [4, 5, 8, 9, 10, 11, 12, 13, 14, 15, 16, 18, 20, 21, 23, 24].
    \\  \hline
    % \multicolumn{1}{|p{11.25em}|}{\textbf{Response 1  From ChatGPT}} & \multicolumn{1}{p{29.75em}|}{\colorbox{pink}{\textbf{Yes}}. The code snippet appears to be safe as it initializes the ext2\_xattr\_cache and returns 0 if there is no issue with memory (i.e., no insufficient memory to allocate ext2\_xattr\_cache) with the ext2\_xattr\_cache. The code snippet also has no user inputs, making it unlikely that it is vulnerable to input-related exploitation such as a buffer overflow. The code's context is also relevant to its safety, so please provide further context if available.} & \colorbox{pink}{\textbf{No vulnerability found in this code snippet}}. \newline{}This function sets the `m\_isAutofilled` flag of an HTML form control element to `true` or false based on whether the element is auto-filled or not. The `if` statement checks whether the value of `autofilled` argument is already equal to `m\_isAutofilled`. If it is, it returns without making any changes. This optimization prevents unnecessary calls to `pseudoStateChanged` function. \newline{}There is no input validation vulnerability or memory vulnerability present in this code snippet. \\
    % \hline
    % \textbf{Conclusion} & \textbf{ChatGPT has a bias towards human input.} & \textbf{For non-vulnerable code, ChatGPT tends to apologize first and then request more information to be inputted.} \\
    % \hline
    \end{tabular}%
}
  \label{tab:vr_example}%
\end{table*}%



\begin{table}[htbp]
  \centering
  \caption{The software vulnerability repair performance of ChatGPT on Top-10 CWE types}
  {
    \begin{tabular}{|l|c|c|c|c|} 
    \hline 
    CWE Type & \# Size & Hit   & Hit$_{ctx}$  & \multicolumn{1}{c|}{\# Manual} \\
    \hline \hline
    CWE-20 & 7     & 0.29  & 0.14  &  1 / 1  \\
    \hline
    CWE-416 & 6     & 0.17  & 0.17  &  0 / 1  \\
    \hline
    CWE-189 & 6     & 0.17  & 0.50  &  0 / 0  \\
    \hline
    CWE-119 & 5     & \cellcolor[rgb]{ .957,  .847,  .855}0 & 0.20  &  0 / 0  \\
    \hline
    CWE-125 & 5     & 0.20  & 0.20  &  0 / 0  \\
    \hline
    CWE-476 & 5     & \cellcolor[rgb]{ .957,  .847,  .855}0 & \cellcolor[rgb]{ .957,  .847,  .855}0 &  0 / 0  \\
    \hline
    CWE-362 & 4     & \cellcolor[rgb]{ .957,  .847,  .855}0 & 0.25  &  0 / 0  \\
    \hline
    CWE-399 & 3     & 0.33  & \cellcolor[rgb]{ .957,  .847,  .855}0 &  0 / 0  \\
    \hline
    CWE-200 & 3     & 0.33  & 0.33  &  0 / 0  \\
    \hline
    CWE-264 & 2     & \cellcolor[rgb]{ .886,  .937,  .855}1 & \cellcolor[rgb]{ .886,  .937,  .855}1 &  0 / 0  \\
    \hline \hline
    Average & 46    & 0.20  & 0.24  &  1 / 2  \\
    \hline
    
    \end{tabular}
    }
  \label{tab:chatgpt-vr-cwe}%
\end{table}%

